Tiny Machine-Learning Operations within Cyber-Physical Systems: a Field Study

Machine-Learning Operations (MLOps) is maturing into a software-engineering discipline, yet its tiny-scale variant (TinyMLOps)-targeting the resource-constrained microcontrollers embedded in cyber-physical systems (CPS)-remains poorly understood in industrial practice. Opaque models, noisy heterogeneous data, and tight memory budgets hinder adoption in safety-critical settings, where most decisions still rely on human experts. We report a field study of an end-to-end, knowledge-centered TinyMLOps pipeline that fuses domain physics, expert speculation, and sensor streams to deliver explainable, low-footprint models deployable on-device. The pipeline spans automated collection and cleaning of heterogeneous time series, knowledge-driven feature construction, interpretable regularized models, and rolling temporal cross-validation under concept drift. We evaluate it on 4.4 GB of data from two offshore-wind cable-trenching campaigns. The classifier anticipates harmful load peaks up to three minutes ahead at 0.84 AUC within a 32 kB footprint on an ARM Cortex-M4; an ablation shows that injecting prior knowledge halves false alarms and surfaces actionable operational rules. Replaying recommendations in operational dashboards indicates an 11% reduction in non-productive time. We distill engineering lessons and validity threats for trustworthy TinyMLOps in CPS, and release code and an annotated dataset to support reproducibility.

==> App/08_LoadPeaksSouthFork.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/Load Peak identifier 0 Southfork.png}
    \caption{ACG Load Peak Classification per Cable for South Fork: Part 1}
    \label{fig:LoadPeakIdentifierSouthFork1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/Load Peak Identifier 16 Southfork.png}
    \caption{ACG Load Peak Classification per Cable for South Fork: Part 2}
    \label{fig:LoadPeakIdentifierSouthFork2}
\end{figure}

==> App/08_soilDensityCohesivenessParameters.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/rq2_layer0.png}
    \caption{Fitted Coefficients of Soil Layer 0 Proportion (of ACG) on Probability of Peak. }
    \label{fig:LayerCoefficients0}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/rq2_layer1.png}
    \caption{Fitted Coefficients of Soil Layer 1 Proportion (of ACG) on Probability of Peak. }
    \label{fig:LayerCoefficients1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/rq2_layer2.png}
    \caption{Fitted Coefficients of Soil Layer 2 Proportion (of ACG) on Probability of Peak. }
    \label{fig:LayerCoefficients2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/rq2_layer3.png}
    \caption{Fitted Coefficients of Soil Layer 3 Proportion (of ACG) on Probability of Peak. }
    \label{fig:LayerCoefficients3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/08_RQ2/rq2_layer4.png}
    \caption{Fitted Coefficients of Soil Layer 4 Proportion (of ACG) on Probability of Peak. }
    \label{fig:LayerCoefficients4}
\end{figure}


==> App/08_southForkSoilLayers.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{l p{5.6cm}}
\toprule
Soil Layer ID & Soil Layer Name \\
\midrule
L00         & L01 - SAND - Gravelly - Very loose to loose       \\
L01         & L02 - SAND - Gravelly - Medium dense to dense     \\
L02         & L03 - SAND - Very gravelly - Very dense           \\
L03         & L04 - SAND - Silty - Medium dense to dense        \\  
L04         & L05 - SILT - Clayey - Low to medium strength      \\
L05         & L06 - SILT - Clayey - High to very high strength  \\    
L06         & L07 - SAND - Gravelly - Medium dense to dense     \\
L07         & L08 - SILT - Clayey - High to very high strength  \\
L08         & L08 - BASE                                        \\
\bottomrule
\end{tabular}
\end{table}

==> App/1_kaskasiIntervals.tex <==
% ==================================================
%                     Appendix A
% ==================================================
\begin{figure}
    \centering
    \includegraphics[width=.41\textwidth]{Fig/03_caseStudy/kaskasiMapMPs.png}
    \caption{Kaskasi Node Overview}
    \label{fig:kaskasiMapMPs}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=.41\textwidth]{Fig/app/kaskasiCableDurations.png}
    \caption{Kaskasi Cable Trenching Intervals}
    \label{fig:kaskasiCableDurations}
\end{figure}
%
\csvautotabular{Data/kaskasiCableDuration.csv}



==> App/2_kaskasiSoilLayers.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{l p{5.6cm}}
\toprule
Soil Layer ID & Soil Layer Name \\
\midrule
L00         & Sandy SILT Low to medium strength             \\
L01         & Silty SAND Very loose to loose                \\
L02         & Gravelly SAND Medium dense to dense           \\
L03         & Silty CLAY Low to medium strength             \\  
L04         & SAND Medium dense to dense                    \\
L05         & SAND Dense to very dense                      \\    
L06         & SAND Medium dense to dense                    \\
L07         & Silty SAND Medium dense to dense              \\
L08         & clayey SILT High to very high strength        \\
L09         & SAND Dense to very dense                      \\
\bottomrule
\end{tabular}
\end{table}

==> App/3_loadPeaks.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 0.png}
    \caption{ACG Load Peak Classification per Cable: Part 1}
    \label{fig:LoadPeakIdentifier1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 8.png}
    \caption{ACG Load Peak Classification per Cable: Part 2}
    \label{fig:LoadPeakIdentifier2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 16.png}
    \caption{ACG Load Peak Classification per Cable: Part 3}
    \label{fig:LoadPeakIdentifier3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 24.png}
    \caption{ACG Load Peak Classification per Cable: Part 4}
    \label{fig:LoadPeakIdentifier4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 32.png}
    \caption{ACG Load Peak Classification per Cable: Part 5}
    \label{fig:LoadPeakIdentifier5}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Fig/app/Load Peak Identifier 40.png}
    \caption{ACG Load Peak Classification per Cable: Part 6}
    \label{fig:LoadPeakIdentifier6}
\end{figure}


==> Ch/14_biographies.tex <==
% ==================================================
%                   Author Biographies
% ==================================================
% NOTE TO AUTHORS: TSE biographies have three paragraphs (education;
% employment & research interests; society memberships, service, awards).
% Please complete the bracketed degree/year/institution details before
% submission, and REMOVE this whole file for the blinded manuscript.

\begin{IEEEbiographynophoto}{Damian A. Tamburri}
received the Ph.D. degree in computer science from VU University Amsterdam,
The Netherlands.

He is an Associate Professor with the University of Sannio, Italy, and with
JADS/NXP Semiconductors. His teaching and research span big-data engineering,
deep learning, and AI engineering, with a focus on the software engineering of
data- and ML-intensive systems, MLOps, and socio-technical aspects of software
development.

He is an Editorial Board Member of ACM TOSEM and IEEE Transactions on Services
Computing, secretary of the OASIS TOSCA Technical Committee, and secretary of
the IFIP Working Groups (TC2, TC6, TC8) on Service-Oriented Computing.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Willem-Jan van den Heuvel}
received the Ph.D. degree in information systems from Tilburg University,
The Netherlands.

He is a Professor of data engineering with Tilburg University and the Jheronimus
Academy of Data Science (JADS). His research interests include data engineering,
service-oriented and cloud computing, and the engineering of data-intensive and
ML-based enterprise systems.

He has served on the program committees of numerous international conferences and
journals in services, cloud, and data engineering.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jaymon Veldkamp}
received the M.Sc. degree in Data Science in Business and Entrepreneurship from
the Jheronimus Academy of Data Science (JADS)/Tilburg University,
The Netherlands.

His work, conducted in collaboration with an industrial partner in offshore
marine engineering, focuses on knowledge and data engineering, MLOps, and the
application of explainable machine learning to cyber-physical systems.

His professional interests include data-driven decision support for industrial
operations and the deployment of machine learning on resource-constrained
embedded devices.
\end{IEEEbiographynophoto}

